Incremental Risk Assessment for Cascading Failures in Large-Scale Multi-Agent Systems

We develop a framework for studying and quantifying the risk of cascading failures in time-delay consensus networks, motivated by a team of agents attempting temporal rendezvous under stochastic disturbances and communication delays. To assess how failures at one or multiple agents amplify the risk of deviation across the network, we employ the Average Value-at-Risk as a systemic measure of cascading uncertainty. Closed-form expressions reveal explicit dependencies of the risk of cascading failure on the Laplacian spectrum, communication delay, and noise statistics. We further establish fundamental lower bounds that characterize the best-achievable network performance under time-delay constraints. These bounds serve as feasibility certificates for assessing whether a desired safety or performance goal can be achieved without exhaustive search across all possible topologies. In addition, we develop an efficient single-step update law that enables scalable propagation of conditional risk as new failures are detected. Analytical and numerical studies demonstrate significant computational savings and confirm the tightness of the theoretical limits across diverse network configurations.

==> extra_content.tex <==

% \subsubsection{Proof of Lemma \ref{lem:sig_star}}
% The proof is an direct result of Lemma \ref{lem:y_steady} by considering the eigenvalues of the star graph topology $\lambda_i = 1$ for any $i \in \{ 2, \dots, n - 1\}$ and $\lambda_n = n$. The general expression (after some basic algebraic calculations) can be written as
% \begin{align*}
%     \sigma_{ij} 
%     &= \frac{1}{2} b^2 \bigg(g(\tau) \big((QQ^T)_{ij} - (\bm{q}_1\bm{q}_1^T)_{ij} - (\bm{q}_n\bm{q}_n^T)_{ij} \big) \\
%     & \hspace{2cm} + \dfrac{1}{n} g(n \tau)(\bm{q}_n\bm{q}_n^T)_{ij}\bigg)
% \end{align*}
% where $g(x)$ is as defined in $\eqref{eq:g}$
% For the case of $i \neq j$ and all $i, j \in \{ 1, \dots, n - 1\}$ 
% \begin{align*}
%     \sigma_{ij} 
%     &= \frac{1}{2} b^2 \bigg(g(\tau) \bigg(0 - \dfrac{1}{n} - \dfrac{1}{n(n-1)} \bigg) + \dfrac{1}{n} g(n \tau)\dfrac{1}{n(n-1)} \bigg)
% \end{align*}
% The result follows by simplification.\\
% The result for other cases follows similarly by considering the fact that $Q$ is an orthogonal matrix and using appropriate elements of the matrices $(\bm{q}_1\bm{q}_1^T)$ and $(\bm{q}_n\bm{q}_n^T)$ .
% \hfill$\square$

% \subsubsection{Proof of Lemma \ref{lem:star_mu_sig}}
% The proof is similar to the proof of Lemma \ref{lem:complete_mu_sig_cond} by taking appropriate elements of covariance matrix for the agents on the periphery and the agents on the center. The result follows by basic algebraic calculations
% \hfill$\square$

% \subsubsection{Proof of Lemma \ref{lem:star_mu_sig_2}}
% The proof is similar to the proof of Lemma \ref{lem:complete_mu_sig_cond}. The $\tilde{\Sigma}_{22}^{-1}$ is calculated using the inverse formula involving Schur complement. The result follows by basic algebraic manipulations.  
% \hfill$\square$

% \subsubsection{Proof of Theorem \ref{thm: exptd_value}}:
% For brevity, let $\rho' = \sqrt{1 - \rho^2}$
% \begin{align*}
%      \mathbb{E}_Q[y_j| y_i \in U_{\delta_i}]=  \frac{\mathbb{E}_Q[y_j \mathbf{1}_{y_i \in U_{\delta_i}}]}{\mathbb{E}_Q[\mathbf{1}_{y_i \in U_{\delta_i}}]}\\
%     = \frac{\int_{-\infty}^{\infty}\int_{-\infty}^{y^*}\frac{y_je^{-\frac{1}{2 \rho'^2}\big[ \rho'^2 \big(\frac{y_j}{\sigma_j}\big)^2 + \big(\frac{y_i}{\sigma_i} - \rho \frac{y_j}{\sigma_j}\big)^2\big]} dy_i dy_j}{2\pi \sigma_j\sigma_i \rho'} }{\int_{-\infty}^{y^*} \frac{1}{\sqrt{2 \pi} \sigma_i} e^{-\big(\frac{y_i}{\sigma_i}\big)^2}}\\
%     = \frac{\int_{-\infty}^{\infty}y_j \frac{e^{-\frac{1}{2 } \big(\frac{y_j}{\sigma_j}\big)^2}}{\sqrt{2 \pi} \sigma_j}  \frac{1}{2}\big[1 + erf\big[ \frac{y^* - \rho \frac{\sigma_i}{\sigma_j}y_j}{\sqrt{2}\rho'\sigma_i}\big] \big] dy_j}{\frac{1}{2}\big[1 + erf\big[ \frac{y^*}{\sqrt{2}\sigma_i}\big] \big]}
% \end{align*}
%  The last step involves the application of Fubini's theorem \cite{durrett2019probability} to split the double integral into iterated integral. It is trivial to verify that the conditions for Fubini's Theorem are satisfied by the integrand. It is straightforward to see that the term $\int_{-\infty}^{\infty}y_j \frac{e^{-\frac{1}{2}\big(\frac{y_j}{\sigma_j}\big)^2}}{\sqrt{2 \pi} \sigma_j} dy_j$ in the numerator is 0 as it represents expected value of univariate Gaussian random variable with mean 0. 
%  % In order to write the algebraic expressions in compact form, we introduce following notations, $\alpha_1 = \frac{1}{2\sigma_j^2}$, $\beta = \frac{y^*}{\sqrt{2}\rho' \sigma_i}$, $\alpha_2 = \frac{\rho}{\sqrt{2}\rho' \sigma_j}$
% %  \begin{align*}
% %      \mathbb{E}_Q[y_j| y_i \in \mathcal{W}_i]
% %     &= \frac{\frac{\int_{-\infty}^{\infty}y_j e^{- a_1 y_j^2} erf(\beta - a y_j)}{\sqrt{2 \pi} \sigma_j}dy_j}{\big[1 + erf\big[ \frac{y^*}{\sqrt{2}\sigma_i}\big] \big]}
% % \end{align*}
% % Using the following result for $a_1 > 0, a\geq 0$ \cite{korotkov2020_error}
% The result follows by using the integral solution in \cite{korotkov2020_error}
% % $$
% % \int_{-\infty}^{\infty}z e^{- a_1 z^2} erf(a z + \beta)dz =\frac{a}{a_1 \sqrt{a^2 + a_1}}e^{-\frac{a_1 \beta^2}{a^2 + a_1}} 
% % $$
% % It is straightforward to see that in our case , coefficient $-a>0$ for $\rho <0$. The result follows by simple algebraic calculation. For $\rho\geq0$, we use the property of error function being odd to get the coefficient $a \geq 0$. The result then follows by similar calculations.
 
%  \subsubsection{Proof of Lemma \ref{lem: sup_exptd_value}}:
% Since, $\sigma_i$ and $\sigma_j$ varies with $g^2$
% it is straightforward to analyze that 
% $$\mathbb{E}_\mathbb{Q}[y_j | y_i \in \mathcal{W}_{\delta_i}] = -\frac{\rho}{\sqrt{2 \pi}}\frac{\sigma_j e^{\frac{-\rho^2y^{*2}}{2 \sigma_i^2}}}{1 + erf(\frac{y^*}{\sqrt{2} \sigma_i})} $$
% % is monotonically increasing in $g.$ 
% is monotonic function in $g$ depending on sign of  $\rho$. 
% The result then follows by substituting the smallest or the largest value of $g $ depending on sign of $\rho$. The bound follows similarly.

% Since, $\sigma_i$ and $\sigma_j$ varies with $g^2$, it is straightforward to see  $$\mathbb{E}_\mathbb{Q}[y_j | y_i \in \mathcal{W}_{\delta_i}] = \frac{|\rho|}{\sqrt{2 \pi}}\frac{\sigma_j e^{\frac{-\rho^2y^{*2}}{2 \sigma_i^2}}}{1 + erf(\frac{y^*}{\sqrt{2} \sigma_i})} $$ 


% is monotonic function in $g$ depending on sign of  $\rho$. 
% The result then follows by substituting the smallest or the largest value of $g = g_0 (1 + \epsilon)$ depending on $\rho$. The bound follows similarly.

n other words, when formulating cascading failure for agent $j$, it is assumed that agent $i$ has failed to reach the $c$-consensus. We study the conditional statistics of the steady-state observable of the $j$'th agent, which is represented by $\bar{y}_j|\bar{y}_{i} = y_f$ for some $|y_f| > c$. 

\begin{lemma}   \label{lemma:single_conditional_prob}
    For every two steady-state observables $\bar{y}_i$ and $\bar{y}_{j}$, given that $\bar{y}_{i} = y_f$, the conditional distribution of $\bar{y}_{j}$ is a normal distribution $\mathcal{N}(\tilde{\mu},\tilde{\sigma}^2)$, where
    $$
    \tilde{\mu} = \rho_{ij} \frac{\sigj}{\sigi} y_f,
    \text{ and }
    ~ \tilde{\sigma}^2 = \sigj^2 (1 - \rho_{ij}^2),$$ 
    in which $\rho_{ij} = \sigma_{ij} / \sigma_{i} \sigma_{j}$ and $|\rho_{ij}| < 1$ for all $i,j \in \{1,\dots, n\}$ and $i \neq j$. The value of $\sigma_{ij}, \sigma_{i}, \text{ and }\sigma_{j}$ are computed as in \eqref{eq:sigma_y}.
\end{lemma}

The above lemma provides the statistics of the observables with the existence of a large fluctuation in the consensus network. Observing \eqref{eq:sigma_y}, one can find out that the cross-correlation $\rho_{ij}$ is independent to $b$, the magnitude of external noises. This observation implies that the probabilistic inter-relation between two agents originated from the time-delay and the communication graph but not the stochastic perturbation.

Following the notation of Lemma \ref{lemma:single_conditional_prob}, the main scenario assumes that the $i$'th agent fails to achieve the $c$-consensus with $|y_f| > c$ and we study the risk of failure for the $j$'th agent given the previous event.  To measure the risk of cascading failure, we consider the event of failing to reach the $c-$consensus for observable $\bar{y}_{j}$ as 
\begin{align*}
    \Big\{ \bar{y}_{j} \in U_{\delta} \Big\} \text{ with } U_{\delta}=\left( -\infty, -\delta - c\right) \bigcup \left(  \delta+c  ,\infty \right),
\end{align*}
where $c, \delta \in \R_{+}$. It should be noted that in our definition of $U_\delta$ for $c$-consensus, the family of $U_\delta$ obviously depends on $c$ but its dependency to this parameter is omitted from $U_\delta$ for notational simplicity. The associated risk measure is obtained with the conditional probability distribution of $\bar{y}_{j}$, which assumes the $i$'th agent has deviated from the rendezvous time, i.e., $\bar{y}_{i} = y_f$ and $|y_f| > c$. The value-at-risk measure for cascading failure is defined as

\begin{align}\label{eq:single_var}
    \cass = \inf \big\{ \delta > 0 \;\big|\; \mathbb{P} \{ \bar{y}_{j} \in U_{\delta} \;\big|\; \bar{y}_i = y_f\} < \varepsilon \big\},
\end{align}
where the confidence level $\varepsilon$ takes value in $(0,1)$. The value of $\cass$ measures the chance of an agent failing to reach the $c-$consensus given that another agent has failed. $\cass$ takes value in $[0,\infty]$, and the case $\cass = 0$ indicates the scenario when the probability of the cascading failure on the $j$'th agent is always less than $\varepsilon$. The larger the value of $\cass$, the higher the chance of cascading failure is going to occur in the system. The value of $c$ will also play the role as a design parameter when $\cass = 0$ since the system will reach the $c-$consensus with the probability at least $1-\varepsilon$. For the exposition of the next result, we introduce the following notation:
$$
\kappa_{\delta,\pm}^{(i,j)} = \frac{(\delta+c)\sigi^2 \pm \sigma_{ij} y_f}{\sigi\sqrt{2(\sigj^2\sigi^2-\sigma^2_{ij})}}
$$
with $\sigi, \sigj, \sigma_{ij}$ defined in \eqref{eq:sigma_y} and $\kappa_{\delta,\pm}^{(i,j)}$ is a function of $\delta$. The following notation is also introduced for simplicity,
\begin{align} \label{eq:single_S}
    S(\delta) = \inf \left\{ \delta > 0 ~\Big|~ \text{erf}(\kappa_{\delta,+}^{(i,j)}) + \text{erf}(\kappa_{\delta,-}^{(i,j)}) > 2 (1- \varepsilon) \right\}.
\end{align}

\begin{lemma} \label{lem:single_cas_ren_risk}
    Suppose that the consensus network reaches the steady-state and the $i$'th agent has failed to reach the $c$-consensus with the observable $\bar{y}_{i} = y_f$. The risk of cascading large fluctuation at the $j$'th agent is 
    \[
        \cass=\begin{cases}
            0, &\text{if} ~ 1 - \frac{1}{2}\left(\text{erf}(\kappa_{0,+}^{(i,j)}) + \text{erf}(\kappa_{0,-}^{(i,j)}) \right) \leq \varepsilon\\
            S(\delta), &\text{otherwise} 
            \end{cases}
    \]
    where $i, j \in \{1, \dots, n\}$ with $i \neq j$, $|y_f| > c$, and $S(\delta)$ is defined in \eqref{eq:single_S}.
\end{lemma}

Given the $i$'th agent has failed to reach $c$-consensus, one can formulate the risk profile of the network by stacking up all the cascading risk $\cass$ among remaining agents with a systemic risk profile vector $\bm{\mathcal{R}}^{i}_{\varepsilon} \in \R^{n}$ as follows
\begin{equation*}
    \bm{\mathcal{R}}^{i}_{\varepsilon} = \big[\mathcal{R}^{i,1}_{\varepsilon},\dots , \mathcal{R}^{i,n}_{\varepsilon} \big]^T,
\end{equation*}
where $\cass = 0$ if $j = i$.

For the exposition of our next result, we introduce the notation for simplicity:
$$\eta_{\varepsilon_\pm}^{i,j} = \frac{\mathcal{R}_{\varepsilon}^{i,j} + c \pm \Tilde{\mu}}{2\Tilde{\sigma}}$$

% $\Tilde{\mathcal{R}_{\varepsilon}}_- = \frac{\mathcal{R}_{\varepsilon} + c - \Tilde{\mu}}{2\Tilde{\sigma}}$
\begin{theorem} \label{thm:cas_ren_risk_avar}
    Suppose that the consensus network reaches the steady-state and the $i$'th agent has failed to reach the $c$-consensus with the observable $\bar{y}_{i} = y_f$. The average value at risk of cascading large fluctuation at the $j$'th agent is 
    \begin{align*}
        \mathcal{A}_{\varepsilon}^{i,j}&= \dfrac{\Tilde{\sigma}}{\sqrt{2\pi}\varepsilon}\left(e^{-\eta_{\varepsilon_-}^{i,j^2}}  + e^{-\eta_{\varepsilon_+}^{i,j^2}} \right)+\\&
    \hspace{2cm}\dfrac{\Tilde{\mu}}{2\varepsilon}\left( \textup{erf}(\eta_{\varepsilon_+}^{i,j} ) -
    \textup{erf}(\eta_{\varepsilon_-}^{i,j}) \right) - c
       \end{align*}
    % where $i, j \in \{1, \dots, n\}$ with $i \neq j$, $|y_f| > c$, and $S(\delta)$ is defined in \eqref{eq:S}.
\end{theorem}

\subsubsection{Single Existing Failure}

The results above can be applied with Lemma \ref{lem:single_cas_ren_risk} to obtain the closed-from representation of $\cass$. One should notice that, when using the complete graph, the cross-correlation $\rho_{ij} = \frac{-1}{n-1}$, which is uniform for all $i \neq j$. This observation can also be found in Fig. \ref{fig:single_cas_risk}. Let us denote the branch limit in Lemma \ref{lem:single_cas_ren_risk} with the following expression
\begin{equation} \label{eq:zeta}
    \zeta_{\delta,\pm} =\frac{(n-1)(\delta+c) \pm y_f}{\bar{\sigma}\sqrt{2n(n-2)}},
    % \zeta_{\delta,-} =\frac{(n-1)(\delta+c) - y_f}{\bar{\sigma}\sqrt{2n(n-2)}},
\end{equation}
where $\bar{\sigma} = \sigi$ for all $i = {1,\dots,n}$. Then, the risk of cascading large fluctuation $\cass$ can be computed by letting $\kappa_{\delta,+}^{(i,j)} = \zeta_{\delta,+}$ and $\kappa_{\delta,-}^{(i,j)} = \zeta_{\delta,-}$. We also observe the existence of fundamental limits on the diagonal elements of the covariance matrix $\Sigma$.

\subsection{The Path Graph}
If a team of $n$ agents is using an unweighted path graph for communication, which contains $n$ nodes and $n-1$ edges. The eigenvalues are: $\lambda_j = 2(1-cos(\pi(j-1)/n))$, and their corresponding eigenvectors are shown by $\bm{q}_1 = \frac{1}{\sqrt{n}} \bm{1}_n$ and $\bm{q}_k = [q_k^{(1)}, \dots, q_k^{(n)}]^T$ with
$$
q_k^{(l)} = \sqrt{\frac{2}{n}} \cos \left( \frac{\pi(n-j+1)}{2n} (2l-1) \right)
$$
for all $k \in \{2, \dots, n\}$ and $l \in \{1, \dots, n\}$. Then, closed-form cascading risk $\cass$ and $casm$ is immediate by using the computed $\lambda_k$ and $\bm{q}_k$ with Lemma\ref{lem:single_cas_ren_risk} and Lemma\ref{lem:mul_cas_ren_risk} respectively.

% The elements of the covariance matrix are
% \begin{equation*}
%     \sigma_{ij} = \frac{4 g^2 \tau^{3}}{n\pi} \sum_{k=2}^{n} \theta(i,j,k)  f(\lambda_k \tau, \beta \tau),
% \end{equation*}
% in which $\theta(i,j,k) = \sin (\frac{\pi(n-k+1)}{n} i) \sin (\frac{\pi(n-k+1)}{n} j)$ $\sin^2 (\frac{\pi(n-k+1)}{2n})$. Then the cascading risk $\casr$ is immediate following by using Theorem \ref{thm:cas_ren_risk}. 

\subsection{The p-Cycle Graph}
If a network of agents is using $p-$cycle graph for communication, which denotes each vehicle communicates to its $p-$immediate neighbors. From \cite{gray2006toeplitz, van2010graph}, one can show that eigenvalues of the corresponding Laplacian matrix are $\lambda_1 = 0$ and 
$$
\lambda_k = \frac{\sin((2p+1)(k-1)\pi/n)}{\sin((k-1)\pi/n)} - 1.
$$ 
Their corresponding eigenvectors are shown by $\bm{q}_1 = \frac{1}{\sqrt{n}} \bm{1}_n$ and $\bm{q}_k = [q_k^{(1)}, \dots, q_k^{(n)}]^T$ with 
$$
q_k^{(l)} = 2p+1 - \frac{\sin((2p+1)(l-1)\pi/n)}{\sin((l-1)\pi/n)},
$$ 
for all $k \in \{2, \dots, n\}$ and $l \in \{1, \dots, n\}$. Then, one can compute $\cass$ and $\casm$ with the same lines of argument.

% The elements of the covariance matrix $\Sigma$ is shown by
% \begin{equation*}
%     \sigma_{ij} = \frac{g^2 \tau^{3}}{2\pi} \sum_{k=2}^{n} \big(q_k^{(i+1)} - q_k^{(i)} \big) \big( q_k^{(j+1)} - q_k^{(j)} \big)  f(\lambda_k \tau, \beta \tau),
% \end{equation*}
% then one can easily compute the $\casr$ as in Theorem \ref{thm:cas_ren_risk}.

% \subsection{The Complete Graph}
% For a team of agents adopting an unweighted complete communication graph, the eigenvalues of the corresponding Laplacian matrix are: $\lambda_1 = 0$ and $\lambda_j = n$ for all $j = 2,\dots,n$. Then, one can find the closed-form representation for the statistics of steady-state observable $\bar{\bm{y}}$ as follows.

% \begin{lemma} \label{lem:sig_complete}
%     For a team of agents adopting the complete graph with their steady-states observables $\bm{\bar{y}} \sim \mathcal{N}( 0, \Sigma)$, the elements of its covariance matrix $\Sigma$ is shown by
%     \[
%         \sigma_{ij} = 
%         \begin{cases}
%             \dfrac{n-1}{2n^2} \dfrac{\cos (n \tau) \, b^2}{1 - \sin (n\tau)}, &\text{ if } \; i = j\\[10pt]
%             -\dfrac{1}{2n^2}\dfrac{\cos (n \tau) \, b^2}{1 - \sin (n\tau)}, &\text{ if } \; i \neq j\\
%         \end{cases}
%     \]
%     for all $i, j = 1,\dots,n$.
% \end{lemma}

% \begin{lemma} \label{lem:complete_mu_sig_cond}
% Under the assumptions of Lemma \ref{lem:sig_complete}, the conditional distribution of $\bar{y}_j$ conditioned on $m$ existing failures is  $\bar{y}_j \sim \mathcal{N}(\hat{\mu},\hat {\sigma}^2)$ with 
%     \begin{equation}    \label{eq:cond_complete}
%         \hat{\mu} = \frac{- \mathbf{1}_{m}^T \bm{y}_f}{n-m}~~ \text{and}~~\hat{\sigma} = \sigj\sqrt{1 - \frac{m}{(n-1)(n-m)}}.   
%     \end{equation}
% \end{lemma}

% The results above can be applied with Lemma \ref{lem:mul_cas_ren_risk} to obtain the closed-from representation of $\casm$. One should notice that, when using the complete graph, the cross-correlation $\rho_{ij} = \frac{-1}{n-1}$, which is uniform for all $i \neq j$. This observation can also be found in Fig. \ref{fig:mul_cas_risk}. Let us denote the branch limit in Lemma \ref{lem:mul_cas_ren_risk} with the following expression
% \begin{equation} \label{eq:zeta}
%     \zeta_{\delta,\pm} =\frac{(n-1)(\delta+c) \pm y_f}{\bar{\sigma}\sqrt{2n(n-2)}},
%     % \zeta_{\delta,-} =\frac{(n-1)(\delta+c) - y_f}{\bar{\sigma}\sqrt{2n(n-2)}},
% \end{equation}
% where $\bar{\sigma} = \sigi$ for all $i = {1,\dots,n}$. Then, the risk of cascading large fluctuation $\cass$ can be computed by letting $\kappa_{\delta,+}^{(i,j)} = \zeta_{\delta,+}$ and $\kappa_{\delta,-}^{(i,j)} = \zeta_{\delta,-}$. We also observe the existence of fundamental limits on the diagonal elements of the covariance matrix $\Sigma$.



% \subsection{Star Communication Graph}
% We label the agent in the center as the $n$'th agent and the rest of the agent on the periphery are labelled from $1, \dots, n-1 $. The eigenvalues of the corresponding Laplacian matrix are: $\lambda_1 = 0$, $\lambda_j = 1$ for all $j = 2,\dots,n - 1$ and $\lambda_n = n$. The star graph offers the same sparsity as the path graph or the $1-$cycle graph. However, unlike the path graph or the ring graph, the star graph stays connected even if some of the agents on the periphery are disconnected. For the exposition of our next result, we introduce the following notation:
% \begin{equation} \label{eq:g}
%      g(x)  =\frac{\cos{x}}{(1 - \sin{x})}.
% \end{equation}
% Then, the closed-form expression for the steady-state statistics of the observables $\bar{\bm{y}}$ is shown as follows.

% \begin{lemma} \label{lem:sig_star}
%     Suppose that the consensus network \eqref{eq:dyn} with the star communication graph reaches the steady-state, then the statistics of observables follows $\bm{\bar{y}} \sim \N(0, \Sigma)$, in which its covariance matrix $\Sigma$ is given element-wise by\\
%     \[
%         \sigma_{ij} := 
%         \begin{cases}
%             \frac{b^2}{2n (n-1)}\big( n(n-2) g(\tau) + \frac{1}{n} g(n\tau)\big), &\text{ if } \; i = j\\[10pt]
%             \frac{b^2}{2n (n-1)}\big(-n g(\tau) + \frac{1}{n} g(n\tau)\big), &\text{ if } \; i \neq j\\
%         \end{cases}
%     \]
%     for all $i, j = 1,\dots,n - 1$ and
%         \[
%         \sigma_{in} := 
%         \begin{cases}
%             \frac{b^2 (n - 1)}{2n^2} g(n\tau), &\text{ if } \; i = n\\[10pt]
%           \frac{- b^2}{2n^2} g(n\tau), &\text{ if } \; i \neq n\\
%         \end{cases}
%     \]
% \end{lemma}
% For the exposition of our next result, let us consider $\Delta = n^2(n - m - 1) g(\tau) + m g(n\tau)$
% \begin{lemma} \label{lem:star_mu_sig}
%     The conditional distribution of $\bar{y}_j$ considering $m$ existing failures of agents on periphery in a star graph is given by $\bar{y}_j \sim \N(\hat{\mu},\hat {\sigma}^2)$, such that
%             \[
%         \hat{\mu}_i := 
%             \begin{cases}
%             \frac{- (n - 1) g(n\tau)}{\Delta } \mathbf{1}_{m}^T \bm{y}_f, &\text{ if } \; i = n\\[15pt]
%             \frac{\big(- n^2 g(\tau) + g(n\tau)\big)}{\Delta } \mathbf{1}_{m}^T \bm{y}_f, &\text{ if } \; i \neq n\\
%         \end{cases}
%     \]
%     and 
%                 \[
%         \hat{\sigma}_i^2 := 
%             \begin{cases}
%             \sigma_n^2\frac{n^2 (n - m - 1) g(\tau)}{\Delta}, &\text{ if } \; i = n\\[15pt]
%             \frac{b^2 g(\tau)}{2}\bigg(1 + \frac{g(n\tau)}{\Delta }\bigg), &\text{ if } \; i \neq n\\
%         \end{cases},
%     \]
%   %  , \text{ and }~ ~\hat{\sigma} = \sigj\sqrt{1 - \frac{m}{(n-1)(n-m)}},
% where $\bm{1}_m \in \R^m$ is the vector of all ones and $\bm{y}_f$ is the vector of observable of the existing failures.
% \end{lemma}


% \begin{lemma} \label{lem:star_mu_sig}
%     The conditional distribution of $\bar{y}_j$ considering $m - 1$ existing failures of agents on periphery and the failure of the agent in center in a star graph is given by $\bar{y}_j \sim \N(\hat{\mu},\hat {\sigma}^2)$, such that
%     $$ \hat{\mu} = \frac{- \mathbf{1}_{m}^T \bm{y}_f}{n-m}, \text{ and }~ ~\hat{\sigma}^2 = \frac{1}{2} b^2 g(\tau) \bigg(1 - \frac{1}{n-m}\bigg), $$
%   %  , \text{ and }~ ~\hat{\sigma} = \sigj\sqrt{1 - \frac{m}{(n-1)(n-m)}},
%     where $\bm{1}_m \in \R^m$ is the vector of all ones and $\bm{y}_f$ is the vector of observables of existing failures with the observable of the $n$-th, i.e., the central agent being $\bm{y}_f(m)$.
% \end{lemma}


% \subsection{The Path Graph}
% If a team of $n$ agents is using an unweighted path graph for communication, which contains $n$ nodes and $n-1$ edges. The eigenvalues are: $\lambda_j = 2(1-cos(\pi(j-1)/n))$, and their corresponding eigenvectors are shown by $\bm{q}_1 = \frac{1}{\sqrt{n}} \bm{1}_n$ and $\bm{q}_k = [q_k^{(1)}, \dots, q_k^{(n)}]^T$ with
% $$
% q_k^{(l)} = \sqrt{\frac{2}{n}} \cos \left( \frac{\pi(n-j+1)}{2n} (2l-1) \right)
% $$
% for all $k \in \{2, \dots, n\}$ and $l \in \{1, \dots, n\}$. Then, closed-form cascading risk $\cass$ is immediate by using the computed $\lambda_k$ and $\bm{q}_k$ with Lemma\ref{lem:single_cas_ren_risk}.

% The elements of the covariance matrix are
% \begin{equation*}
%     \sigma_{ij} = \frac{4 g^2 \tau^{3}}{n\pi} \sum_{k=2}^{n} \theta(i,j,k)  f(\lambda_k \tau, \beta \tau),
% \end{equation*}
% in which $\theta(i,j,k) = \sin (\frac{\pi(n-k+1)}{n} i) \sin (\frac{\pi(n-k+1)}{n} j)$ $\sin^2 (\frac{\pi(n-k+1)}{2n})$. Then the cascading risk $\casr$ is immediate following by using Theorem \ref{thm:cas_ren_risk}. 

% \subsection{The p-Cycle Graph}
% If a network of agents is using $p-$cycle graph for communication, which denotes each vehicle communicates to its $p-$immediate neighbors. From \cite{gray2006toeplitz, van2010graph}, one can show that eigenvalues of the corresponding Laplacian matrix are $\lambda_1 = 0$ and 
% $$
% \lambda_k = \frac{\sin((2p+1)(k-1)\pi/n)}{\sin((k-1)\pi/n)} - 1.
% $$ 
% Their corresponding eigenvectors are shown by $\bm{q}_1 = \frac{1}{\sqrt{n}} \bm{1}_n$ and $\bm{q}_k = [q_k^{(1)}, \dots, q_k^{(n)}]^T$ with 
% $$
% q_k^{(l)} = 2p+1 - \frac{\sin((2p+1)(l-1)\pi/n)}{\sin((l-1)\pi/n)},
% $$ 
% for all $k \in \{2, \dots, n\}$ and $l \in \{1, \dots, n\}$. Then, one can compute $\casr$ with the same lines of argument.

% % The elements of the covariance matrix $\Sigma$ is shown by
% % \begin{equation*}
% %     \sigma_{ij} = \frac{g^2 \tau^{3}}{2\pi} \sum_{k=2}^{n} \big(q_k^{(i+1)} - q_k^{(i)} \big) \big( q_k^{(j+1)} - q_k^{(j)} \big)  f(\lambda_k \tau, \beta \tau),
% % \end{equation*}
% % then one can easily compute the $\casr$ as in Theorem \ref{thm:cas_ren_risk}.


% \subsection{Shortest Path Between the Agent and the Existing Failure}

% The impact from the existing large fluctuation shows an obvious correlation to the shortest path \cite{bellman1958routing} between the failure location and the agent of the interest in the communication graph topology, and we refer to Fig. \ref{fig:shortest_path}. This correlation can be traced back from the system dynamics \eqref{eq:dyn} that the graph Laplacian specifies the feedback gain between each pair of two agents for the closed-loop system. The most intuitive observation can be found in an unweighted complete graph such that any two agents (nodes) have the same shortest path, i.e., $1$. As a result, the cascading risk $\cass$ remains the same for a fixed time-delay, shown in Fig. \ref{fig:shortest_path} (d). In unweighted $p$-cycle graphs, $\cass$ shows a growing trend as the shortest path between the $i$'th and the $j$'th agent increases. When the network parameter $p$ increases, the pattern gets closer to the complete graph. 

% The most interesting pattern shows up in an unweighted path graph. When the communication time-delay $\tau$ remains small, the cascading risk $\cass$ tends to increase with the shortest path since the effect from the lagged communication will accumulate over the network. However, when $\tau$ gets large, this accumulation starts to lose the dominating effect, and the riskiest agent starts to appear at the middle level of all possible shortest paths. In other words, as time-delay increases, the safe policy of avoiding the cascading risk changes from staying close to the existing failure to get either close to or far from the failure as much as possible.

% \begin{figure}[t]
%     \begin{subfigure}[t]{.49\linewidth}
%         \centering
%     	\includegraphics[width=\linewidth]{Figs/path_tau_single_failure.jpg}
%     	\caption{The path Graph.}
%     	\label{fig:risk_collide_50}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.49\linewidth}
%         \centering
%     	\includegraphics[width=\linewidth]{Figs/1cycle_tau_single_failure.jpg}
%     	\caption{The 1-cycle graph.}
%     	\label{fig:risk_collide_path_10}
%     \end{subfigure}
%     \medskip
%     \begin{subfigure}[t]{.49\linewidth}
%         \centering
%     	\includegraphics[width=\linewidth]{Figs/2cycle_tau_single_failure.jpg}
%     	\caption{The 2-cycle graph.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{.49\linewidth}
%         \centering
%     	\includegraphics[width=\linewidth]{Figs/compelete_tau_single_failure.jpg}
%     	\caption{The complete graph.}
%     \end{subfigure}
%     \caption{The above figures depict the relation between $\cass$ and the shortest path between the existing failure location (the $i$'th agent) and the $j$'th agent.}
%     \label{fig:shortest_path}
% \end{figure}

